Ancilia: Scalable Intelligent Video Surveillance for the Artificial Intelligence of Things

With the advancement of vision-based artificial intelligence, the proliferation of the Internet of Things connected cameras, and the increasing societal need for rapid and equitable security, the demand for accurate real-time intelligent surveillance has never been higher. This article presents Ancilia, an end-to-end scalable, intelligent video surveillance system for the Artificial Intelligence of Things. Ancilia brings state-of-the-art artificial intelligence to real-world surveillance applications while respecting ethical concerns and performing high-level cognitive tasks in real-time. Ancilia aims to revolutionize the surveillance landscape, to bring more effective, intelligent, and equitable security to the field, resulting in safer and more secure communities without requiring people to compromise their right to privacy.

==> tabs/SystemComparison2.tex <==
\begin{table}[t]
    \centering
    \caption{System configurations. Number of Cores, number of CUDA Cores, and amount of VRAM is for a single CPU/GPU of the listed type.}
    \label{tab:sys_configs}
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{c||c|c|c}
        %\cellcolor{DarkGray} & \multicolumn{3}{d||}{Processor} & \multicolumn{3}{d}{GPU}  \\ %\cline{2-7}
        \rowcolor{DarkGray} Name & Processor & Cores & Clock Speed \\ 
        \hline \hline
        Server A & 2$\times$ EPYC 7513 & 32 & 2.6 GHz \\
        %Server & 2x EPYC 7282 & 16 & 2.8 GHz & 4x RTX 3090 & 10496 & 24 GB &  &  &  \\
        Server B & 2$\times$ Xeon E5-2640 v4 & 10 & 2.4 GHz \\
        %Server & 2x Xeon Silver 4114 & 10 & 2.2 GHz & P100 & 3584 & 16 GB &  &  &  \\
        Workstation & Threadripper Pro 3975WX & 32 & 3.50 GHz \\
        %Workstation & Threadripper 1920X & 12 & 3.5 GHz & 2x Titan RTX & 4608 & 24 GB &  &  &  \\
        %Workstation & Ryzen 9 3900X & 12 & 3.8 GHz & Titan V & 5120 & 12 GB &  &  &  \\
        %Laptop & Ryzen 9 5900HS & 8 & 3.0 GHz & RTX 3060 & 3840 & 6 GB &  &  &  \\
        \hline
        \rowcolor{DarkGray} & GPU & CUDA Cores & VRAM \\
        \hline \hline
        Server A & 4$\times$ V100 & 5120 & 32 GB  \\
        Server B & 2$\times$ Titan V & 5120 & 12 GB   \\
        Workstation & 3$\times$ A6000 & 10752 & 48 GB  \\        
    \end{tabular}
    %}
\end{table}

==> tabs/videos.tex <==
\begin{table}[h]
    \centering
    \caption{Crowd density in test videos.}
    \begin{tabular}{c|c}
       Crowd Density & Detection per Second \\ \hline
       Normal & 70 \\
       Heavy & 216 \\
       Extreme & 744 \\
    \end{tabular}
    \label{tab:density}
\end{table}

==> tex/Analysis.tex <==
\section{Analysis}\label{sec:Analysis}\



